COMET: Neural Cost Model Explanation Framework

Cost models predict the cost of executing given assembly code basic blocks on a specific microarchitecture. Recently, neural cost models have been shown to be fairly accurate and easy to construct. They can replace heavily engineered analytical cost models used in mainstream compiler workflows. However, their black-box nature discourages their adoption. In this work, we develop the first framework, COMET, for generating faithful, generalizable, and intuitive explanations for neural cost models. We generate and compare COMET's explanations for the popular neural cost model, Ithemal against those for an accurate CPU simulation-based cost model, uiCA. Our empirical findings show an inverse correlation between the prediction errors of Ithemal and uiCA and the granularity of basic block features in COMET's explanations for them, thus indicating potential reasons for the higher error of Ithemal with respect to uiCA.

==> contents/background.tex <==
\section{Cost Models}

Cost Models are static analyzers of programs, which predict their runtime resource requirements, such as their throughput (number of CPU clock cycles taken for program execution), memory consumption, energy consumption, CPU bottlenecks, etc. They are used to guide compiler optimizations towards low resource-consuming, but semantically equivalent programs, by predicting the resource consumption of candidate optimizations. Some commonly used cost models are uiCA~\cite{uica}, LLVM-MCA~\cite{llvm-mca}, IACA~\cite{iaca}, and Ithemal~\cite{ithemal}. These cost models take basic blocks of x86 assembly code (Definition~\ref{def:bb}) as input and predict their resource requirements. 

Cost models have traditionally been \emph{analytical} CPU simulators, which execute a given basic block several times in a loop and return their average performance prediction. 
%These simulators resemble the physical CPU that the cost model is generating timing predictions for. 
Examples of such simulation-based analytical cost models include uiCA, LLVM-MCA, and IACA. 
%
Recently, machine learning has been used for this cost prediction task. The first ML-based cost model, Ithemal, is a hierarchical LSTM model which predicts the throughput of x86 basic blocks. It is trained on the open-source dataset of x86 basic blocks, BHive~\cite{bhive}, which contains the measured throughput values of over 300,000 basic blocks for three microarchitectures: Haswell, Skylake, and Ivy Bridge. 

==> contents/technical1_archive.tex <==

\section{Formalizing cost model explanation}   
In this section, we formalize explanations for x86 cost models and discuss the desirable properties of the explanations. 
Our objective is to develop a black-box explanation framework to explain the behavior of any given x86 cost model. This allows us to juxtapose the cost prediction behavior of both ML-based and analytical cost models and explain even proprietary x86 cost models.  

%To facilitate the explanation of any x86 cost model, even the proprietary models, we develop an explanation framework that requires just query access to the cost model and hence treats the cost model as a black box. 

We first formalize the cost model as a function $\costmodel: B\rightarrow\mathbb{R}^+$, where $B$ is the (discrete) set of all valid basic blocks according to a given Instruction Set Architecture (ISA) and $\mathbb{R}^+$ denotes the set of positive real numbers, as performance parameters are generally positive quantities. %We can treat $\costmodel$ as an infinite look-up table wherein each basic block is mapped to a number in $\mathbb{R}^+$. 
%
%Given the infinite look-up table model for $\costmodel$,
Let $\mathcal{T}\subseteq\mathbb{R}^+$ be a set of desirable cost values, then 
we can partition $B= B_\mathcal{T} \cup B_{\mathcal{T}}'$ where  $B_\mathcal{T}$ is the set of basic blocks $\basicblock$ that have $\costmodel(\basicblock)\in\mathcal{T}$. 
An explanation for the behavior of $\costmodel$ would be the common concepts in basic blocks in $B_\mathcal{T}$ that are not present in the basic blocks in $B_{\mathcal{T}}'$, as they lead to cost predictions in $\mathcal{T}$. For example, consider a very crude throughput-predicting cost model $\costmodel_1$ that assigns a throughput of $2$ cycles iff a basic block has $8$ instructions. If $\mathcal{T} = \{2\}\subset\mathbb{R}^+$, then $B_\mathcal{T}$ will consist of basic blocks with $8$ instructions, $B_\mathcal{T}'$ will consist of all the other basic blocks and hence the explanation of $\costmodel_1$'s behavior for throughput prediction in $\mathcal{T}$ will be the number of instructions being equal to $8$.

While it might be possible for simple cost models such as $\costmodel_1$ to have global concepts for their predictions that can explain the cost for certain $\mathcal{T}$, generally the computations of a cost model is complex and specialized to exploit features of the input basic block. Hence, we focus on generating explanations of cost prediction $\costmodel(\basicblock)$ with respect to a given basic block $\basicblock$. Our explanations should also apply to other basic blocks that have features in common with $\basicblock$ and have similar cost predictions as $\costmodel(\basicblock)$. We specialize $\mathcal{T}$ for explaining $\costmodel(\basicblock)$ as  $\mathcal{T}_{\costmodel,\basicblock} = [max(0, \costmodel(\basicblock)-\epsilon), \costmodel(\basicblock)+\epsilon]$, where $\epsilon\geq 0$ is a small constant. As the concepts represented by our explanations must be specifically present in $\basicblock$, our generated explanations are in the form of a subset of the set of features $\mathcal{P}_{\basicblock}$ of $\basicblock$.

% given the complexity of cost models used within compiler optimizations~\citep{llvm-mca,uica,iaca} that are designed to simulate the CPU's microarchitecture, it is unlikely to get a simple and informative global cost prediction concept for such a cost model. Hence, we scope down our explanations to capture the features that lead to a certain cost prediction for a given basic block $\basicblock$.

% Similar to the global explanations, explanation for the cost prediction by cost model $\costmodel$ for $\basicblock$, $\costmodel(\basicblock)$ will consist of general concepts across basic blocks including $\basicblock$ that lead to a cost prediction of $\costmodel(\basicblock)$. As these concepts must be specifically present in $\basicblock$, they would be a set of features of $\basicblock$.
The smallest tangible units of an x86 basic block are its tokens (opcodes and operands). Hence, we treat the tokens as the basic features of $\basicblock$. Let $\mathcal{P}_\basicblock$ be the set of all basic features and all functions of basic features, which we cumulatively call features, of $\basicblock$. Examples of elements of $\mathcal{P}_\basicblock$ for the input basic block $\basicblock$ in Figure~\ref{fig:overview}(a) are $\text{number of instructions}=4$
% , $\text{instruction 1}:\ $\mintinline{gas}{add rcx, rax}, 
and $\text{opcode of instruction 2}:\ $ \opcolor{mov}. Note that, as $\mathcal{P}_\basicblock$ captures all the features of $\basicblock$, there is a one-to-one correspondence between $\mathcal{P}_\basicblock$ and $\basicblock$. 
% Ideally, we would like to explain $\basicblock$ over $\mathcal{P}_\basicblock$, as then we can expect to get explanations that specifically explain $\costmodel(\basicblock)$, but it may not be practically feasible or desirable to get such specific explanations for $\basicblock$. We explain over $\mathcal{P}_\basicblock$ for the ideal explanations for $\costmodel(\basicblock)$ in Section~\ref{sec:idealexp} and translate $\mathcal{P}_\basicblock$ to a practical set of features of $\basicblock$, $\Hat{\mathcal{P}}_\basicblock$, in Section~\ref{sec:practicalexp}. 
The remaining discussion in this paper will describe our approach for generating explanations for the cost model $\costmodel$ when predicting the cost for a basic block $\basicblock$. To simplify notation, when it is clear from the context, we will omit $\costmodel$ and $\basicblock$ from the subscripts of symbols, e.g.,$\Hat{\mathcal{P}}_\basicblock$ will be written as $\Hat{\mathcal{P}}$. 

%\todo{make better}



% In this section, we discuss the desired properties of explanations for the local behavior of a given cost model $\costmodel$ around a target basic block $\basicblock$. Let $\mathcal{P}_\basicblock$ be the exhaustive set of predicates corresponding to the features of $\basicblock$. A predicate is a boolean function that evaluates to true when the corresponding feature is present in the $\basicblock$. Thus, $\mathcal{P}_\basicblock$ is the subset of all possible basic block predicates that evaluate to true for $\basicblock$. Note that, $\mathcal{P}_\basicblock$ may not be tractable or expressible in closed form, but forms the basis of our analysis and explanation framework. For example, some elements of $P_\basicblock$ for the basic block in Figure~\ref{fig:overview} are the predicates corresponding to the features \{Instruction 3, data-dependency between instructions 1 and 2, number of instructions in the basic block\}. 
% Let $B$ denote all the possible x86 basic blocks that adhere to the x86 Instruction Set Architecture. 
% %
% The task of explaining the local behavior of $\costmodel$ for $\basicblock$ is then to identify the set of predicates, $\mathcal{F}_{\costmodel,\basicblock}\subseteq \mathcal{P}_\basicblock$, that lead to the throughput prediction $\costmodel(\basicblock)$. 

\subsection{Ideal black-box explanations for $\costmodel(\basicblock)$}\label{sec:idealexp}

Let the set of features $\mathcal{F}^*\subseteq \mathcal{P}$ be the ideal explanation for $\costmodel(\basicblock)$.
The desirable properties of $\mathcal{F}^*$ are that it should be \emph{faithful} to $\costmodel(\basicblock)$, \emph{generalizable} across multiple basic blocks, and be \emph{simple} to comprehend~\citep{explanationprops}. We formalize these notions next. 

% \emph{faithful} to $\costmodel(\basicblock)$, \emph{generalizable} across multiple basic blocks, and \emph{simple} to comprehend. We formalize these notions next. 

Let $\pertmodel:\wp(\mathcal{P})\rightarrow \wp(B)$ be a perturbation function that is given a set of features of $\basicblock$ as input, $\mathcal{F}\in\wp(\mathcal{P})$, and returns a set of basic blocks $B_{\mathcal{F}}\subseteq B$ where each basic block $\basicblock'\in B_{\mathcal{F}}$ differs from $\basicblock$ by some perturbations to the features in $\mathcal{P}\setminus\mathcal{F}$ in $\basicblock$. Consider the example basic block in Figure~\ref{fig:overview}. If $F =$ \{instruction 4: \opcolor{pop} \regcolor{rbx}\}, then the basic block $\basicblock'$ with instructions 1 and 4, shown in Figure~\ref{fig:overview}(e) and other instructions deleted (perturbed) is an element of $B_{\mathcal{F}}$. 

% where each member of $B_{\basicblock}$ contains $F_\basicblock$. 
% $\basicblock'$ would thus have perturbations to only the features in $\mathcal{P}_\basicblock\setminus\mathcal{F}_\basicblock$ in $\basicblock$. \todo{constrain this to be stronger}


\textbf{Faithfulness}.
$\mathcal{F}^{*f}\subseteq \mathcal{P}$ will be faithful to the cost prediction of $\costmodel(\basicblock)$ if perturbations to only the features in $\mathcal{P}\setminus\mathcal{F}^{*f}$ in $\basicblock$ can change the cost prediction of $\costmodel$ by atmost $\epsilon$. \eqref{eq:faithful} presents the condition  $\varphi(\mathcal{F})$ that must hold for faithful explanation $\mathcal{F}^{*f}$. 
\begin{equation}
    \label{eq:faithful}
    \varphi(\mathcal{F}) \triangleq 
    (\mathcal{F}\subseteq\mathcal{P})\wedge
    (\forall\alpha\in \pertmodel(\mathcal{F})\ldotp \costmodel(\alpha) \in\mathcal{T})
\end{equation}

% This implies that the presence of the predicates in $\mathcal{F}^*_{\costmodel,\basicblock}$ can faithfully explain $\costmodel(\basicblock)$, as all the basic blocks $\basicblock'$ in a local region of basic blocks $B_\basicblock$ that have $\mathcal{F}^*_{\costmodel,\basicblock}$ have similar $\costmodel(\basicblock')$ in $\mathcal{B}(\costmodel(\basicblock),r)$, an$r(\approx 0)$ radius ball around $\costmodel(\basicblock)$. 

A trivial, faithful set of features $\mathcal{F}^{*f}$ is $\mathcal{P}$, as $\pertmodel(\mathcal{P}) = \{\basicblock\}$ and $\costmodel(\basicblock)\in\mathcal{T}$. 
But this explanation is not useful, as $P$ can faithfully explain $\basicblock$ for any cost model but it does not capture the specific behavior of a given $\costmodel$ for predicting the cost of $\basicblock$.   

%does not generalize across different basic blocks and hence does not capture $\costmodel$'s behavior. %Hence, we need generalizability of cost model explanations as a desirable property, which we describe next. 

\textbf{Generalizability and Simplicity of explanations}. %\todo{check for correctness: check introduced due to clustering of bbs point}
To overcome the above issue, we require that faithful explanations of $\basicblock$, $\mathcal{F}^{*f}$ should also apply to other blocks which contain the features in $\mathcal{F}^{*f}$ and where $\costmodel$ makes predictions similar to $\costmodel(\basicblock)$ (generalizable).
% To have higher utility, the ideal explanation $\mathcal{F}^*_{\costmodel,\basicblock}$ should be able to faithfully explain and hence generalize across the maximum number of basic block clusters which include the basic blocks $\alpha$ for which $\mathcal{F}^*_{\costmodel,\basicblock}\subseteq\mathcal{P}_{\alpha}$. 
Every set $\mathcal{F}\subseteq\mathcal{P}$ will have a corresponding set of basic blocks (potentially empty), $\Omega_{\mathcal{F}}$~\eqref{eq:maxgenset} containing basic blocks having the features in $\mathcal{F}$ as faithful explanations where $\costmodel$'s predictions are similar. 
% Let us denote this set as . 
% Let $\mathcal{F}^{*fg}_{\costmodel,\basicblock}$ be an ideal faithful and most generalizable explanation.  
For the faithful explanations with maximum generalizability, $\mathcal{F}^{*fg}$, we need to maximize the cardinality of $\Omega_{\mathcal{F}}$ over the set of faithful explanations $\mathcal{F}^{*f}$. 
% and hence solve the optimization problem in~\eqref{eq:maxgeneralize}.
% number of basic blocks $\alpha$ that have $\mathcal{F}^{*fg}_{\costmodel,\basicblock}$ as faithful explanations. %, and hence maximize $B_{\mathcal{F}^{*fg}_{\costmodel,\basicblock}}$. 
% Thus, we need to solve the optimization problem in~\eqref{eq:maxgeneralize} to obtain $\mathcal{F}^{*fg}_{\costmodel,\basicblock}$. 
% As basic blocks are composed of discrete elements, the cardinality of $B_{\mathcal{F}_{\costmodel,\basicblock}}$, $\mid B_{\mathcal{F}_{\costmodel,\basicblock}}\mid$ is a valid expression. 
% i.e. $\mathcal{F}^*_{\costmodel,\basicblock}$ must satisfy~\eqref{eq:generalize}, where $B'\subseteq \pertmodel_\basicblock(\mathcal{F}^*_{\costmodel,\basicblock})$. 
\begin{equation}
    \label{eq:maxgenset}
    \Omega_{\mathcal{F}} \triangleq \{\alpha\mid \alpha\in\pertmodel(\mathcal{F})\text{ and }\costmodel(\alpha)\in\mathcal{T} \text{ and }\mathcal{F}_{\alpha}^{*f} = \mathcal{F}\}
\end{equation}
% \begin{equation}
%     \label{eq:maxgeneralize}
%     \mathcal{F}^{*fg} \triangleq \mathop{argmax}_{\mathcal{F}\mid\varphi(\mathcal{F})}  \lvert \Omega_{\mathcal{F}}\rvert
% \end{equation}

%
% \textbf{Simplicity of explanations}. 
To have higher interpretability, the ideal explanation $\mathcal{F}^*$ should be simple. While there can be many metrics for simplicity of explanations, a valid metric for explanation sets over $\mathcal{P}$ is the cardinality of $\mathcal{F}^*$~\citep{explanationsize,interpretmlbook}.
% Another valid simplicity metric is the simplicity of features identified in the explanation. We can rank the features in $\mathcal{P}_\basicblock$ according to their simplicity, where more high-level features can be called simpler as compared to low-level features. Possible examples of low-level features could be the individual tokens of $\basicblock$, examples of features that are higher level than tokens could be the individual instructions of $\basicblock$, and even higher-level features of $\basicblock$ could be the number of instructions in $\basicblock$. As the features become simpler, they become more interpretable, but they might get too abstracted away from $\basicblock$. For example, in the basic block $\basicblock$ in Figure~\ref{fig:overview}, the number of instructions = 4 feature can be true for many basic blocks which are very different in terms of their throughput prediction than $\costmodel(\basicblock)$, while the presence of instruction 1 in another basic block might not make it very different from $\basicblock$. For a feature $f\in\mathcal{P}_\basicblock$, we define $Simplicity(f) = $ \todo{add the simplicity of predicates as an optimization objective}
% define the simplicity of a feature $f$ in $\mathcal{P}_\basicblock$ by the level to which $\basicblock$ should be abstracted to make $f$ a \todo{higher-order/higher-level features} 
Hence, to obtain simple, faithful, and generalizable explanations $\mathcal{F}^{*}$, we solve the optimization problem~\eqref{eq:overallideal}, where $\lambda > 0$ is a regularization parameter. 
% \begin{equation}
%     \label{eq:simple}
%     \mathcal{F}^{*fs}_{\costmodel,\basicblock} = \mathop{argmin}_{\mathcal{F}_{\costmodel,\basicblock}\mid \varphi(\mathcal{F}_{\costmodel,\basicblock})} \lvert \mathcal{F}_{\costmodel,\basicblock}\rvert  
% \end{equation}

  
\begin{equation}
    \label{eq:overallideal}
    \mathcal{F}^* \triangleq \mathop{argmax}_{\mathcal{F}\mid \varphi(\mathcal{F})} (\lvert \Omega_{\mathcal{F}}\rvert - \lambda.\lvert \mathcal{F}\rvert)
\end{equation}


% \textbf{Necessity of explanations}.
% Let $\mathcal{F}^{*n}_{\costmodel,\basicblock}\subseteq \mathcal{P}_{\basicblock}$ denote a set of features that are necessary to explain $\costmodel(\basicblock)$. Thus, if the features in $\mathcal{F}^{*n}_{\costmodel,\basicblock}$ are not present in $\basicblock'$, then $\costmodel(\basicblock')\not\in\mathcal{T}_{\costmodel,\basicblock}$. 

% \textbf{Faithfulness}. 
% $\mathcal{F}^{*f}_{\costmodel,\basicblock}\subseteq \mathcal{P}_{\basicblock}$ will be locally faithful to the throughput prediction of $\costmodel(\basicblock)$ iff the presence of $\mathcal{F}^{*f}_{\costmodel,\basicblock}$ results in $\costmodel(\basicblock)$ and any perturbations to predicates in $\mathcal{P}\setminus\mathcal{F}^{*f}_{\costmodel,\basicblock}$ can change the throughput predictions of $\costmodel$ by atmost $\epsilon\approx 0, \epsilon\geq 0$. \eqref{eq:faithful} presents the formula $\varphi(\mathcal{F}^{*f}_{\costmodel,\basicblock})$ that must hold for locally faithful explanation $\mathcal{F}^{*f}_{\costmodel,\basicblock}$. $\mathcal{B}(\costmodel(\basicblock),\epsilon)$ in~\eqref{eq:faithful} denotes an $\epsilon$ radius ball around $\costmodel(\basicblock)$. 
% \begin{equation}
%     \label{eq:faithful}
%     \varphi(\mathcal{F}^{*f}_{\costmodel,\basicblock}) \equiv (\mathcal{F}^{*f}_{\costmodel,\basicblock}\subseteq\mathcal{P}_{\basicblock})\wedge(\forall\basicblock'\in \pertmodel_\basicblock(\mathcal{F}^{*f}_{\costmodel,\basicblock})\ldotp \costmodel(\basicblock') \in\mathcal{B}(\costmodel(\basicblock),\epsilon))
% \end{equation}
% \todo{give an example}
% This implies that the presence of the predicates in $\mathcal{F}^*_{\costmodel,\basicblock}$ can faithfully explain $\costmodel(\basicblock)$, as all the basic blocks $\basicblock'$ in a local region of basic blocks $B_\basicblock$ that have $\mathcal{F}^*_{\costmodel,\basicblock}$ have similar $\costmodel(\basicblock')$ in $\mathcal{B}(\costmodel(\basicblock),r)$, an$r(\approx 0)$ radius ball around $\costmodel(\basicblock)$. 

% Given the complexity of cost models, \eqref{eq:faithful} may be unsatisfiable. In order to make the problem of identifying explanations for cost models satisfiable, we can make two simplifications to~\eqref{eq:faithful}. First, we can require $\costmodel(\basicblock')\in\mathcal{B}(\costmodel(\basicblock),r)$, where $\mathcal{B}(\costmodel(\basicblock),r)$ is a $r(\approx 0)$ radius ball around $\costmodel(\basicblock)$. Second, instead of requiring that all $\basicblock'\in B$ which satisfy the predicates in $\mathcal{F}^*_{\costmodel,\basicblock}$ have similar $\costmodel(\basicblock')$, we can restrict to all $\basicblock'\in B_\basicblock$, where $B_\basicblock\subseteq B$ is a local region of $\basicblock$ in $B$. The former requirement over $B$ requires $\mathcal{F}^*_{\costmodel,\basicblock}$ to explain the behavior of $\costmodel$ globally but $\mathcal{F}^*_{\costmodel,\basicblock}$ may not be able to capture the complete highly non-linear behavior of $\costmodel$ faithfully. On the other hand, restricting to a local region $B_\basicblock$ of $\basicblock$ requires $\mathcal{F}^*_{\costmodel,\basicblock}$ to explain the local behavior of $\costmodel$, which be more closely approximated, making $\mathcal{F}^*_{\costmodel,\basicblock}$ more faithful to $\costmodel(\basicblock)$. Therefore, \eqref{eq:faithful} gets modified to~\eqref{eq:faithful1}. 
% \begin{equation}
%     \label{eq:faithful1}
%     \widetilde{\varphi}(\mathcal{F}^*_{\costmodel,\basicblock}) = \forall\basicblock'\in B_\basicblock\ldotp  \mathcal{F}^*_{\costmodel,\basicblock}\subseteq\mathcal{P}_{\basicblock'}\Leftrightarrow\costmodel(\basicblock')\in\mathcal{B}(\costmodel(\basicblock),r)
% \end{equation}

% \textbf{Generalizability}.
% To have higher utility, the ideal explanation $\mathcal{F}^*_{\costmodel,\basicblock}$ should be able to generalize across the maximum number of basic blocks $\basicblock'$ for which $\mathcal{F}^*_{\costmodel,\basicblock}\subseteq\mathcal{P}_{\basicblock'}$. For the faithful explanations that generalize the most, we would need to solve the optimization problem in~\eqref{eq:maxgeneralize}, where $B_{\mathcal{F}_{\costmodel,\basicblock}}$ is the set of basic blocks that satisfy the predicates in $\mathcal{F}_{\costmodel,\basicblock}$ for which $\costmodel$'s behavior is explained by $\mathcal{F}_{\costmodel,\basicblock}$~\eqref{eq:maxgenset}. As basic blocks are composed of discrete elements, the cardinality of $B_{\mathcal{F}_{\costmodel,\basicblock}}$, $\mid B_{\mathcal{F}_{\costmodel,\basicblock}}\mid$ is a valid expression. 
%i.e. $\mathcal{F}^*_{\costmodel,\basicblock}$ must satisfy~\eqref{eq:generalize}, where $B'\subseteq \pertmodel_\basicblock(\mathcal{F}^*_{\costmodel,\basicblock})$. 
% \begin{equation}
%     \label{eq:maxgenset}
%     B_{\mathcal{F}_{\costmodel,\basicblock}} = \{\alpha\mid \alpha\in\pertmodel_\basicblock(F_{\costmodel,\basicblock})\text{ and } \mathcal{F}_{\costmodel,\widetilde{\basicblock}}^{*f} = \mathcal{F}_{\costmodel,\basicblock}\}
% \end{equation}
% \begin{equation}
%     \label{eq:maxgeneralize}
%     \mathcal{F}^{*fg}_{\costmodel,\basicblock} = \mathop{argmax}_{\mathcal{F}_{\costmodel,\basicblock}\mid\varphi(\mathcal{F}_{\costmodel,\basicblock})}  \lvert B_{\mathcal{F}_{\costmodel,\basicblock}}\rvert
% \end{equation}

% \begin{equation}
%     \label{eq:maxgeneralize}
%     \mathcal{F}^*_{\costmodel,\basicblock} = \mathop{argmax}_{F_{\costmodel,\basicblock}\mid\ \forall \widetilde{\basicblock}\in B' . \mathcal{F}^*_{\costmodel,\basicblock'} = \mathcal{F}^*_{\costmodel,\basicblock}} \lvert B'\rvert
% \end{equation}


% \textbf{Simplicity of explanations}. 
% To have higher interpretability, the ideal explanation $\mathcal{F}^*_{\costmodel,\basicblock}$ should be simple. While there can be many metrics for simplicity of explanations, for the explanation set derived from the basic block features' predicate set $\mathcal{P}_\basicblock$, a valid simplicity metric is the cardinality of $\mathcal{F}^*_{\costmodel,\basicblock}$. Hence, for enhanced simplicity of faithful explanations $\mathcal{F}^{*fs}_{\costmodel,\basicblock}$, we solve the optimization problem~\eqref{eq:simple}. 
% \begin{equation}
%     \label{eq:simple}
%     \mathcal{F}^{*fs}_{\costmodel,\basicblock} = \mathop{argmin}_{\mathcal{F}_{\costmodel,\basicblock}\mid \varphi(\mathcal{F}_{\costmodel,\basicblock})} \lvert \mathcal{F}_{\costmodel,\basicblock}\rvert
% \end{equation}



\subsection{Practical black-box explanations for $\costmodel(\basicblock)$}\label{sec:practicalexp}

There are two levels of intractability in the above formulation of ideal explanations~\eqref{eq:overallideal}. First, the evaluation of the faithfulness condition~\eqref{eq:faithful} for a given set of features $\mathcal{F}$ requires querying $\costmodel$ for the cost prediction of all the basic blocks in the large set, $\pertmodel(\mathcal{F})$. We refer the reader to Appendix~\ref{app:samplespacesize} for examples of some estimates of the cardinality of $\pertmodel(\mathcal{F})$ for different $\basicblock$ and $\mathcal{F}$. Second, the evaluation of the generalizability of $\mathcal{F}$ by the computation of the set $\Omega_{\mathcal{F}}$ requires predicting the cost $\costmodel(\alpha)$ and computing faithful explanations $\mathcal{F}_{\alpha}^{*f}$ for all basic blocks in $\pertmodel(\mathcal{F})$. Hence to make the explanation problem practically solvable, we relax the problem as we describe next.

% The optimization problem in~\eqref{eq:overallideal} can be unsolvable in a reasonable amount of time as it is conditioned on $\varphi(\mathcal{F}_{\costmodel,\basicblock})$ which has a universal quantifier\todo{cite smt solving where univ quant is hard, inf num of bbs} and also involves finding faithful explanations for all the basic blocks $\alpha$ in $\pertmodel_\basicblock(F_{\costmodel,\basicblock})$ to compute $B_{\mathcal{F}_{\costmodel,\basicblock}}$, which again require the satisfaction of $\varphi(\mathcal{F}_{\costmodel,\alpha})$. 
% Hence to make the problem practically solvable, we introduce some approximations which we describe in this section. \todo{2 levels of intractability}

\textbf{Probabilistic faithfulness of explanations}. 
% Consider the notion of faithfulness of explanations, obtained by the satisfaction of $\varphi(\mathcal{F})$ in~\eqref{eq:faithful}. 
To simplify the evaluation of $\varphi(\mathcal{F})$ in~\eqref{eq:faithful} for a given set of features $\mathcal{F}\subseteq\mathcal{P}$, we relax the requirement of the throughput prediction for all $\basicblock'\in\pertmodel(\mathcal{F})$ to be in $\mathcal{T}$ with the requirement that $Pr_{\basicblock'\sim\mathcal{D}_\mathcal{F}}(\costmodel(\basicblock')\in\mathcal{T})\geq(1-\delta)$, where $(1-\delta)$ is the confidence with which our explanations are faithful ($0\leq\delta\leq1$) and $\mathcal{D}_{\mathcal{F}}$ is a basic block distribution over $\pertmodel(\mathcal{F})$.  
%


We identify that $Pr_{\basicblock'\sim\mathcal{D}_{\mathcal{F}}}(\costmodel(\basicblock')\in\mathcal{T})$ is analogous to the notion of \emph{precision}~\eqref{eq:precision} used in prior work~\citep{anchors}, and hence we adopt this terminology.  
Thus, probabilistic faithful explanations $\Hat{\mathcal{F}}^{*f}$ must satisfy the condition $\hat{\varphi}(\mathcal{F})$, given by~\eqref{eq:probfaithful}. 

\begin{equation}
    \label{eq:precision}
    Prec(\mathcal{F}) \triangleq Pr_{\basicblock'\sim\mathcal{D}_{\mathcal{F}}}(\costmodel(\basicblock')\in\mathcal{T})
\end{equation}
\begin{equation}
    \label{eq:probfaithful}
    \hat{\varphi}(\mathcal{F}) \triangleq (\mathcal{F}\subseteq\mathcal{P})\wedge(Prec(\mathcal{F})\geq(1-\delta))
\end{equation}
As $\mathcal{D}_{\mathcal{F}}$ should be such that $\hat{\varphi}(\mathcal{F})$ closely approximates the ideal faithfulness condition $\varphi(\mathcal{F})$~\eqref{eq:faithful} where there is no prioritization over the basic blocks in $\pertmodel(\mathcal{F})$, $\mathcal{D}_{\mathcal{F}}$ should ideally be a uniform distribution over $\pertmodel(\mathcal{F})$ and hence depend on $\basicblock$ and $\mathcal{F}$. 
% $\pertmodel_\basicblock(\mathcal{F}_{\costmodel,\basicblock})$ depends on $\basicblock$ and $\mathcal{F}_{\costmodel,\basicblock}$ and hence   

\textbf{Probabilistic generalizability and simplicity of explanations}. 
% Given a set of (probabilistically) faithful explanations $\Hat{\mathcal{F}}^{*f}_{\costmodel,\basicblock}$, we might not be able to efficiently compute $B_{\Hat{\mathcal{F}}^{*f}_{\costmodel,\basicblock}}$, i.e. the set of basic blocks in $\pertmodel_\basicblock(\Hat{\mathcal{F}}^{*f}_{\costmodel,\basicblock})$ for which $\Hat{\mathcal{F}}^{*f}_{\costmodel,\basicblock}$ is a probabilistic faithful explanation, and hence the maximization problem in~\eqref{eq:maxgeneralize} might not be solvable. 
We relax the requirement of the conditions in the computation of $\Omega_{\mathcal{F}}$~\eqref{eq:maxgenset} and hence maximize the cardinality of $\pertmodel(\mathcal{F})$ over the set of (probabilistically) faithful explanations instead. 

% Thus, we relax~\eqref{eq:maxgeneralize} to~\eqref{eq:probmaxgeneralize}. 
% \begin{equation}
%     \label{eq:probmaxgeneralize}
%     \Hat{\mathcal{F}}^{*fg} \triangleq \mathop{argmax}_{\mathcal{F}\mid\varphi(\mathcal{F})}  \lvert \pertmodel(\mathcal{F})\rvert
% \end{equation}
Note that $\pertmodel$ is a monotonically decreasing function (proof in Appendix~\ref{app:proionofs}). 
Thus, we can get simple explanations with minimum $\lvert\mathcal{F}\rvert$ by 
maximizing $\lvert\pertmodel(\mathcal{F})\rvert$. 
We identify that $\lvert \pertmodel(\mathcal{F})\rvert/\lvert \pertmodel(\emptyset)\rvert$ (where $\emptyset$ denotes the empty set of features) is analogous to the notion of \emph{coverage} in prior work~\citep{anchors}, and hence we adopt this terminology. $Cov(\mathcal{F})$ essentially denotes the fraction of the set of all valid perturbations of $\basicblock$ (which is a fixed set for a given $\basicblock$) that retain the features in $\mathcal{F}$. Note that, $Cov(\mathcal{F})$ is well-defined as $\pertmodel$ is monotonically decreasing which implies that $\pertmodel(\mathcal{F})\subseteq\pertmodel(\emptyset)$. We further relax coverage to denote the probability of observing all the features in $\mathcal{F}$ in an arbitrary valid perturbation of $\basicblock$. ~\eqref{eq:coverage} defines the coverage of a set of features $\mathcal{F}$, defined over a distribution $D$ over the sample space $\pertmodel(\emptyset)$. To obtain an unbiased measure of coverage, $D$ should ideally be a uniform distribution over $\pertmodel(\emptyset)$ which depends on $\basicblock$.  
\begin{equation}
    \label{eq:coverage}
    Cov(\mathcal{F}) \triangleq Pr_{\alpha\sim\mathcal{D}}(\mathcal{F}\in\mathcal{P}_\alpha)
    %\frac{\lvert \pertmodel_\basicblock(\mathcal{F}_{\costmodel,\basicblock})\rvert}{\lvert B\rvert}
\end{equation}

\textbf{Practical set of basic block features}. 
We restrict $\mathcal{P}$, which consists of all features and functions of features of $\basicblock$, to $\Hat{\mathcal{P}}\subset\mathcal{P}$, to reduce the possible sets of features to evaluate in the optimization problem in~\eqref{eq:overallideal}. We define $\Hat{\mathcal{P}}\subset\mathcal{P}$ as the set of features that are actually used in the cost prediction algorithms of popular throughput-predicting cost models such as~\citep{uica,llvm-mca,iaca,ithemal} and hence are interpretable for our stakeholders, i.e. the compiler and performance engineers. 
Hence, our perturbation function $\pertmodel$ also analogously translates to $\Hat{\pertmodel}:\wp(\Hat{\mathcal{P}})\rightarrow\wp(B)$. 
We detail the features in $\Hat{\mathcal{P}}$ in Section~\ref{sec:explanationfeatures}. 

\textbf{Overall optimization problem for practical explanations}. 
Thus, our optimization algorithm to find practically useful explanation concepts $\Hat{\mathcal{F}}^{*}$ for  $\costmodel(\basicblock)$ becomes~\eqref{eq:overallapproxpractical}.
% \todo{add 'such that' condition to the}
\begin{equation}
    \label{eq:overallapproxpractical}
    \Hat{\mathcal{F}}^{*} \triangleq \mathop{argmax}_{\mathcal{F}\mid \mathcal{F}\subseteq\Hat{\mathcal{P}}}  \lvert Cov(\mathcal{F})\rvert \text{ s.t. } Prec(\mathcal{F})\geq(1-\delta)
\end{equation}


% To identify $\mathcal{F}^*_{\costmodel,\basicblock}$, we can consider all the elements $\mathcal{F}\subseteq\wp(\mathcal{P}_{\costmodel,\basicblock})$ (powerset of all predicates), non-deterministically select $\basicblock'$ the features corresponding to $\mathcal{F}$, and if $\costmodel(\basicblock') \neq \costmodel(\basicblock)$, then we can . We select the minimum cardinality set satisfying the requirements for being an explanation, in order to generate more interpretable explanations.
% \[\mathcal{F}^*_{\costmodel,\basicblock} = \mathop{argmin}_{\mathcal{F}\in\wp(\mathcal{P}_{\costmodel,\basicblock}), \costmodel(\basicblock) \Leftrightarrow \overline{\costmodel}(\mathcal{F})} \mid\mathcal{F}\mid\]

% A crucial step in generating $\mathcal{F}^*_{\costmodel,\basicblock}$ is the evaluation of 





==> contents/technical2_archive.tex <==
\begin{figure*}[htb]
    \centering
    \includegraphics[width=\textwidth]{figures/overview.png}
    \caption{\tool{} is given an x86 cost model $\mathcal{M}$ and an x86 basic block $\basicblock$ as input. \tool{} identifies the features of $\basicblock$ that explain the prediction $\costmodel(\basicblock)$. \tool{} first converts $\basicblock$ to a multi-graph $\mathcal{G}$ in (b). $\mathcal{G}$ has the instructions and data dependencies of $\basicblock$ as its vertices and edges respectively. The features $\Hat{\mathcal{P}}$ of $\basicblock$,  are then extracted from $\mathcal{G}$ to give the pool of features in (c). (d) then forms the power set of all the features in $\Hat{\mathcal{P}}$. These sets of features are fed into \tool{}'s perturbation algorithm $\Gamma$ that generates several perturbations $\basicblock'$ that preserve the features in the corresponding (same color) input feature set $\mathcal{F}$ as shown in (e). \tool{} obtains the predictions of cost model $\costmodel$ for each $\basicblock'$, which are then used for the estimation of the precision and coverage of a $\mathcal{F}$. $\mathcal{F}$ having precision higher than $(1-\delta)$ with maximum coverage are output as \tool{}'s explanation for $\costmodel(\basicblock)$ in (f).}
    \label{fig:overview}
\end{figure*}


\section{COMET: Cost Model Explanation Framework}\label{sec:implementation}
This section presents \tool{}, our novel framework for creating practical, black-box, faithful, generalizable, and simple explanations for the predictions made by x86 cost models for a target basic block. 
% \tool{} is a cost-model-agnostic framework that requires just query access to the x86 cost model in order to explain its predictions for a target basic block. 
%\tool{} is especially useful for explaining state-of-the-art ML-based x86 cost models such as Ithemal~\citep{ithemal}, as they are not inherently interpretable.
%
The core operation of \tool{} is to efficiently solve the optimization problem in~\eqref{eq:overallapproxpractical} for a given cost model $\costmodel$ and target basic block $\basicblock$. An overview of \tool{}'s algorithm on an example x86 basic block is shown in Figure~\ref{fig:overview}. To create interpretable explanations, \tool{} first transforms the features/tokens of the input basic block $\basicblock$ into interpretable functions of features that form our $\Hat{\mathcal{P}}$. We detail the algorithm for the construction of the elements of $\Hat{\mathcal{P}}$, which we also call \emph{block features}, in \tool{} in Section~\ref{sec:explanationfeatures}. 
%
After fixing $\Hat{\mathcal{P}}$, we need to evaluate the precision of each subset of $\Hat{\mathcal{P}}$ and identify a subset $\mathcal{F}$ that has $Prec(\mathcal{F})\geq(1-\delta)$ and has maximum $Cov(\mathcal{F})$. To efficiently solve this constrained optimization problem, \tool{} adapts the Anchors explanation algorithm~\citep{anchors}, which has a similar optimization objective, for the x86 cost model explanation setting [Section~\ref{sec:anchoradapt}]. Figure~\ref{fig:overview} presents a simplified overview of \tool{}. 

\subsection{Extracting block features}\label{sec:explanationfeatures}
% To extract useful explanation features, over which \tool{} generates the explanation concepts for $\costmodel(\basicblock)$, 

\tool{} casts the input basic block $\basicblock$ into a multi-graph $\graphbb = (\mathcal{V},\mathcal{E})$, which we describe next. Figure~\ref{fig:overview}(b) shows an example of our formulation. 
%
We define $\mathcal{V}$ as the set of all the instructions in $\basicblock$. There are two types of edges in $\mathcal{E}$: $\mathcal{E}_{seq}$ and $\mathcal{E}_{dep}$. $\mathcal{E}_{seq}$ are the directed edges between the vertices between consecutive instructions, from an instruction to its immediately following instruction. $\graphbb$ can be traversed along the edges in $\mathcal{E}_{seq}$ to obtain the underlying unique basic block $\basicblock$. 

$\mathcal{E}_{dep}$ are the directed, labeled edges corresponding to a data dependency between a pair of instructions. 
While each instruction is processed sequentially by the different components of the CPU, an instruction $\instruction_j$ can get stalled due to the requirement for a previous instruction $\instruction_i$ to get completed, creating a \emph{data dependency hazard}~\citep{comporgdes}. A Read-After-Write (RAW) data-dependency hazard arises when $\instruction_j$ reads the value in an operand that is written by $\instruction_i$. $\instruction_j$ can not get executed until $\instruction_i$ ends to ensure correct execution. 
A Write-After-Read (WAR) hazard occurs when $\instruction_j$ writes to an operand that is read by $\instruction_i$.
A Write-After-Write (WAW) hazard arises when $\instruction_j$ writes to an operand that is written to by $\instruction_i$. 
$\mathcal{E}_{dep}$ consists of directed edges from $\instruction_i$ to $\instruction_j$, labeled by the type of data dependency hazard.
Figure~\ref{fig:overview}(b) shows all the hazards in the example block. 
% For example, the basic block in Figure~\ref{fig:overview}(b) has a RAW hazard between instructions 1 and 2 due to the value in register \textcolor{red}{rcx} being read by instruction 2 after being written in instruction 1, a WAW hazard between instructions 2 and 3 caused by register \textcolor{blue}{rdx} and a WAR hazard between instructions 3 and 4 caused by register \textcolor{ForestGreen}{rdx}. Note that there can be multiple types of data-dependency hazard edges between the nodes corresponding to two instructions in $\basicblock$. We also have a set of sequence edges connecting the nodes corresponding to consecutive instructions in $\basicblock$. $\graphbb(\basicblock)$ can be traversed along these edges between nodes corresponding to consecutive instructions to obtain the underlying unique basic block $\basicblock$. This formulation of $\basicblock$ as $\graphbb(\basicblock)$ enables us to capture the syntactic and semantic features of $\basicblock$, which we use to express our explanations of the throughput prediction for $\basicblock$ by the target cost model. 

% We derive two types of \emph{graph features} from $\graphbb(\basicblock)$: \emph{syntactic} features, $\allfeats_{syntactic}(\basicblock)$ and \emph{semantic} features, $\allfeats_{semantic}(\basicblock)$. This categorization of the graph features $\allfeats(\basicblock)$ enables us to analyze the dependence of a given cost model on the different types of features of $\basicblock$ while making its throughput prediction. Figure~\ref{fig:overview}(c) shows the basic block graph features for the example basic block. 

We derive three types of explanation features of $\basicblock$ from $\graphbb$ to constitute $\Hat{\mathcal{P}}$: instructions ($\mathcal{V}$), data-dependencies ($\mathcal{E}_{dep}$), and number of instructions ($\lvert\mathcal{V}\rvert$). Thus $\Hat{\mathcal{P}} = \mathcal{V}\cup\mathcal{E}_{dep}\cup\{\lvert\mathcal{V}\rvert\}$. Figure~\ref{fig:overview}(c) shows the features in $\Hat{\mathcal{P}}$ for the example basic block. These elements of $\Hat{\mathcal{P}}$ are the features that play a crucial role in the cost prediction algorithms of common models~\citep{uica,ithemal}. %\todo{rephrase to still be model-agnostic}
% As syntactic features, we have features of $\graphbb(\basicblock)$ which do not depend on $\basicblock$'s specific instructions and dependency structures and are general meta-graph properties, such as the number of nodes in the multigraph, which corresponds to the number of instructions in the basic block ($\numinsts(\basicblock)$). \citet{uica} have shown that the number of instructions is an important feature for throughput prediction, and simple functions of the number of instructions in a basic block can lead to a fairly accurate prediction of the throughput for several basic blocks. Hence, $\numinsts(\basicblock)\in\allfeats_{syntactic}(\basicblock)$. 

% As semantic features, we have the nodes and the data-dependency edges of $\graphbb(\basicblock)$, which correspond to $\basicblock$'s instructions ($\allinstructions(\basicblock)$) and data dependencies ($\alldatadependencies(\basicblock)$). These features determine the exact operations performed by $\basicblock$ and hence should be important factors governing its throughput. Thus, $\allinstructions(\basicblock)\cup\alldatadependencies(\basicblock)\in\allfeats_{semantic}(\basicblock)$. 

% \todo{checkout if a note on tokens as features is needed}


\subsection{Efficiently computing explanations}\label{sec:anchoradapt}
% \todo{don't emphasize on estimation: first 2 paras}
% To solve the optimization problem in~\eqref{eq:overallapproxpractical} over $\Hat{\mathcal{P}}$, we need to compute the $Prec(\mathcal{F})$ and $Cov(\mathcal{F})$ of $\mathcal{F}\subseteq\Hat{\mathcal{P}}$ over distributions $\mathcal{D}_{\mathcal{F}}$ and $D$ respectively. 

% Different distributions represent differing prioritizations of basic blocks in $\Hat{\pertmodel}(\mathcal{F})$. 
% As $\Hat{\pertmodel}(\mathcal{F})$ can be infinite and 
To efficiently compute explanations, \tool{} empirically estimates $Prec(\mathcal{F})$ and $Cov(\mathcal{F})$ with samples from $\mathcal{D}_{\mathcal{F}}$ and $D$ respectively. 
%
% Similarly, the coverage $Cov(\mathcal{F})$ which denotes the probability of observing all the features in $\mathcal{F}$ in an arbitrary basic block $\in B$ is defined over an arbitrary distribution $D$ over $B$, which may not be representable in closed form for precise computation of coverage. Hence, for efficiency of explanation computation, we empirically estimate $Cov(\mathcal{F})$ as well. 
% 
% Next, we describe our choice of the distributions $\mathcal{D}_{\mathcal{F}}$ and $D$ and their sampling algorithms in \tool{} with which \tool{} empirically estimates $Prec(\mathcal{F})$ and $Cov(\mathcal{F})$. 
%
% We have designed $\mathcal{D}_{\mathcal{F}}$ to be an (approximately) uniform distribution over $\Hat{\pertmodel}(\mathcal{F})$, as any prioritization of basic blocks can affect the explanation concepts for a cost model in arbitrary ways. 
%
We have designed \emph{basic block perturbation algorithms} to sample from $\mathcal{D}_{\mathcal{F}}$ and $D$, which essentially perturb $\basicblock$ to obtain basic blocks $\basicblock'$ according to the corresponding distribution from the underlying sample space. As discussed in Section~\ref{sec:practicalexp}, we want both $\mathcal{D}_{\mathcal{F}}$ and $D$ to be uniform distributions over $\Hat{\pertmodel}(\mathcal{F})$ and $\Hat{\pertmodel}(\emptyset)$ respectively to compute unbiased relaxations of the ideally desirable explanations. Observe that, $D$ is hence a special case of $\mathcal{D}_{\mathcal{F}}$ with $\mathcal{F} = \emptyset$. 
% Moreover, we want both $\mathcal{D}_{\mathcal{F}}$ and $D$ to be uniform distributions. 
Thus, the perturbation algorithm corresponding to $\mathcal{D}_{\mathcal{F}}$ can be used for $D$ as well. %, by keeping $\mathcal{F} = \emptyset$.  

% We perturb each feature of $\basicblock$ uniformly to make $\basicblock'$ a uniformly selected sample from the underlying distribution. 
% We describe our basic block perturbation algorithm next. 

% Observe that, $\Hat{\pertmodel}(\mathcal{F})\subseteq\Hat{\pertmodel}(\emptyset)$. As $\mathcal{D}_{\mathcal{F}}$ and $D$ are uniform distributions over $\Hat{\pertmodel}(\mathcal{F})$ and $\Hat{\pertmodel}(\emptyset)$ respectively, $\mathcal{D}_{\mathcal{F}} = D_{\basicblock'\mid\mathcal{F}\subseteq\mathcal{P}'}$, i.e. $\mathcal{D}_{\mathcal{F}}$ is a conditional distribution conditioned on having the features $\mathcal{F}$ in the samples. Hence, we develop a common perturbation algorithm for both $\mathcal{D}_{\mathcal{F}}$ and $D$ with the only difference being that we freeze the features in $\mathcal{F}$ in $\basicblock$ while perturbing to obtain a sample from $\mathcal{D}_{\mathcal{F}}$. 



\textbf{Basic block perturbation algorithm}. 
\tool{}'s basic block perturbation algorithm $\Gamma:\wp(\Hat{\mathcal{P}})\rightarrow\Hat{\pertmodel}(\emptyset)$ takes a set of features $\mathcal{F}\in\wp(\Hat{\mathcal{P}})$ as input and randomly perturbs $\basicblock$ to obtain $\basicblock'\in\Hat{\pertmodel}(\mathcal{F})$, $\basicblock'\sim\mathcal{D}_{\mathcal{F}}$ such that $\basicblock'$ retains the features in $\mathcal{F}$ and has some features in $\Hat{\mathcal{P}}\setminus\mathcal{F}$ perturbed to valid values. Figure~\ref{fig:overview}(e) shows examples of perturbations of $\basicblock$ created by $\Gamma$. While we ideally want $\mathcal{D}_{\mathcal{F}}$ to be a uniform distribution over $\Hat{\pertmodel}(\mathcal{F})$, 
$\Hat{\pertmodel}(\mathcal{F})$ is complex without a closed form characterization and is also defined differently for individual $\mathcal{F}$. This makes designing an algorithm to generate uniform samples for each $\Hat{\pertmodel}(\mathcal{F})$ hard. 
We observe that as $\Hat{\pertmodel}(\mathcal{F})$ can be a large set of basic blocks (check Appendix~\ref{app:samplespacesize} to get an idea of the magnitude of these sample spaces), the probability of uniformly sampling a given $\basicblock'\in\Hat{\pertmodel}(\mathcal{F})$ will be very small. 
Hence, we relax the requirement of sampling from a uniform distribution over $\Hat{\pertmodel}(\mathcal{F})$ to the ability of $\Gamma$ to produce diverse basic blocks from $\Hat{\pertmodel}(\mathcal{F})$ so that the probability of perturbing to a given basic block is small. 
% Thus, $\Gamma$ is a randomized perturbation algorithm that employs several heuristics to produce diverse perturbed basic blocks $\basicblock'$. 
%We describe the working of $\Gamma$ to create diverse perturbed basic blocks next. 

$\Gamma$ perturbs $\graphbb = (\mathcal{V},\mathcal{E})$ to obtain $\graphbb' = (\mathcal{V}',\mathcal{E}')$, which uniquely corresponds to $\basicblock'$, such that the features in $\mathcal{F}\subseteq\Hat{\mathcal{P}}$ are preserved.
To obtain $\graphbb'$, % for a given $\mathcal{F}$,
%
% , i.e. the set of features to preserve in $\basicblock'$, some elements of $\graphbb$, which corresponds to the features in $\Hat{\mathcal{P}}\setminus\mathcal{F} = (\mathcal{V}\cup\mathcal{E}_{dep}\cup\{\lvert\mathcal{V}\rvert\})\setminus\mathcal{F}$ are perturbed. Thus, we can perturb some elements in $\mathcal{V}$ and $\mathcal{E}_{dep}$ which do not affect the preservation of the features in $\mathcal{F}$ to get $\basicblock'$. 
%
$\Gamma$ attempts to perturb every element of $\zeta = \mathcal{V}\cup\mathcal{E}_{dep}$ that is allowed to be perturbed, independent of the others. This is because any dependence will restrict the possible choices for $\basicblock'$ and hence disproportionately increase the probabilities of some possible outputs of $\Gamma(\mathcal{F})$. In order to create independence between the elements of $\zeta$, $\Gamma$ perturbs each $v,v'\in\mathcal{V}, v\neq v'$ independent of each other. $\Gamma$ also perturbs $\varepsilon, \varepsilon'\in\mathcal{E}_{dep}, \varepsilon\neq\varepsilon'$ such that $\varepsilon$ and $\varepsilon'$ do not have any vertex in common, independent of each other. However when $\varepsilon$ and $\varepsilon'$ have at least one vertex in common with the corresponding instruction pairs being $(\instruction_{i},\instruction_{j})$ and $(\instruction_j, \instruction_k)$ respectively, if they are caused by a common operand in $\instruction_j$, then all perturbations to $\varepsilon$ and $\varepsilon'$ can not be made completely independent, otherwise they are perturbed independently. 
% Elements $v\in\mathcal{V}$ and $\varepsilon\in\mathcal{E}_{dep}$ are perturbed independently as long as $\varepsilon$ is not an incoming or outgoing edge of $v$. 
For independence between an element $v\in\mathcal{V}$ and $\varepsilon\in\mathcal{E}_{dep}$, $\Gamma$ perturbs only the opcode of the corresponding instruction of $v$ to perturb $v$ and only the operands of the instructions connected by $\varepsilon$ to perturb $\varepsilon$. 
%Note however that certain choices of opcode changes for perturbation of $v$ can inadvertently result in perturbations to $\varepsilon$, but this is block specific. 

$\Gamma$ preserves the instructions corresponding to every data dependency in $\mathcal{F}$. $\Gamma$, however, does not require the data dependencies corresponding to every instruction in $\mathcal{F}$ to stay preserved, as it associates an instruction with its opcode, while data dependencies can be perturbed by operand changes as well. This requires fewer features to be preserved beyond $\mathcal{F}$, increasing the number of choices for $\basicblock'$. 

\emph{Perturbing elements of $\mathcal{V}$}.
$\Gamma$ perturbs an element $v$ of $\mathcal{V}$ by either deleting or replacing it with another valid vertex that corresponds to a valid x86 basic block instruction. The deletion perturbation is permissible when $\lvert\mathcal{V}\rvert\not\in\mathcal{F}$. When $v$ is deleted, all incoming and outgoing edges to $v$ are removed from $\graphbb(\basicblock)$, and a sequence edge is introduced between the vertex preceding and the vertex following $v$. 
In order to replace $v$, the corresponding instruction $\instruction$'s opcode is replaced with another opcode in the x86 Instruction Set Architecture that can produce a valid x86 basic block instruction (an instruction that does not contain certain opcodes such as \opcolor{call} or \opcolor{jmp}) with the operands of $\instruction$. This is done so that the resultant $\basicblock'\in\Hat{\pertmodel}(\emptyset)\subseteq B$. 
% We do not change the operands of $\instruction$ for perturbing $v$ as we account for their changes to perturb data dependencies.  
% changes in operands to be changes in the data-dependency edges in $\graphbb(\basicblock)$ in order to approximately create independence between the graph features. 
%
Overall, $\Gamma$ independently perturbs or retains every $v$ with equal probability, where $v$ is perturbed by either deleting it (when $\lvert\mathcal{V}\rvert\not\in\mathcal{F}$) or replacing $v$ with a valid $v'$, again with equal probability, to obtain $\mathcal{V}'$.

% As $\Hat{\mathcal{P}} = \mathcal{V}\cup\mathcal{E}_{dep}\cup\{\lvert\mathcal{V}\rvert\}$, \tool{} consists of custom perturbation algorithms for $\mathcal{V}$ $\mathcal{E}_{dep}\cup\{\lvert\mathcal{V}\rvert$  

\emph{Perturbing elements of $\mathcal{E}_{dep}$}.
$\Gamma$ perturbs $\varepsilon\in\mathcal{E}_{dep}$ by deleting the corresponding dependency, $\dependency$. 
% While changes to opcodes of instructions corresponding to the data dependency could result in the deletion of the dependency, we consider their changes vertex perturbations. 
$\dependency$ is deleted by perturbing some operands $\gamma$ corresponding to $\dependency$ to other operands of the same type and size as $\gamma$. The type of $\gamma$ would be memory, register, or immediate/constant, while its size could be a power of $2$ between $2^3-2^9$ bits. Hence, we change the operand registers/memory addresses to other registers/memory addresses to break the data dependencies. 
% Note that this change in operands can create new data dependencies in the resulting basic block, but we do not consider these new dependencies as they are not present in $\basicblock$ and hence can not be important features for its throughput predictions. 
%
Overall, $\Gamma$ either perturbs/deletes or retains a data dependency by similar probabilities. The exact probabilities of perturbation and retention will be basic block specific and are discussed in Appendix~\ref{app:pertmodeldetails}.  
% We prioritize the deletion of data-dependency edges in our implementation as they generally result in minor operand changes and prioritizing their deletion can help us expand the high-probability scenario space of our local basic block distribution. We note, however, that \tool{} can be tuned not to prioritize the deletion of the edges in order to obtain a narrower local basic block distribution.


Algorithm~\ref{alg:perturb_bb} in Appendix~\ref{app:pertalgo} presents the pseudocode of $\Gamma$ to 
% (conditionally, for a given $\mathcal{F}$) 
perturb a given basic block $\basicblock$.


% Let $\Gamma:\wp(\Hat{\mathcal{P}})\rightarrow\Hat{\pertmodel}(\emptyset)$ be \tool{}'s perturbation algorithm that takes  $\mathcal{F}\in\wp(\Hat{\mathcal{P}})$ as input and perturbs $\basicblock$ to $\basicblock'\in\Hat{\pertmodel}(\mathcal{F})$ such that $\basicblock'\sim\mathcal{D}_{\mathcal{F}}$. $\Gamma$ generates $\basicblock'$ randomly by independently perturbing the features in $\Hat{\mathcal{P}}\setminus\mathcal{F}$. 

% write how the basic block perturbation algorithm works

% $\Gamma$ first partitions $\Hat{\mathcal{P}}$ into $\mathcal{F}_{retained}$ and $\mathcal{F}_{changed}$, which are the set of features of $\basicblock$ that are retained and changed respectively in $\basicblock'$. $\mathcal{F}_{retained}$ is such that $\mathcal{F}\subseteq\mathcal{F}_{retained}$. The set of features $\mathcal{F}_R = \mathcal{F}_{retained}\setminus\mathcal{F}$ that are preserved alongside $\mathcal{F}$  in $\basicblock'$ are selected randomly and hence vary across every execution of $\Gamma$. 
% The implication of the partitioning is that $\basicblock'\in\Hat{\pertmodel}(\mathcal{F}_{retained})\subseteq\Hat{\pertmodel}(\mathcal{F})$. 
% Hence, we restrict the sampling of $\basicblock'$ to a randomly selected subset of the set of basic blocks from which we have to sample.    
% $\basicblock' = \Hat{\pertmodel}(\mathcal{F}\cup\mathcal{F}_R)\subseteq\Hat{\pertmodel}(\mathcal{F})$. 
% Thus, $\Gamma$ picks $\basicblock'$ from a randomly selected restricted set of basic blocks $\Hat{\pertmodel}(\mathcal{F}'_{\costmodel,\basicblock})$ where $\mathcal{F}'_{\costmodel,\basicblock} = \mathcal{F}\cup\mathcal{F}_R$. 
% Let $\mathcal{F}_R = \mathcal{F}_{dep}\cup\mathcal{F}_{inst}$, where $\mathcal{F}_{dep}$ denotes the dependencies and $F_{inst}$ denotes the instructions in $\mathcal{F}_R$. The probability of selection of  $\mathcal{F}_R$
% , which corresponds to the restricted sampling space $\Hat{\pertmodel}(\mathcal{F}_{retained})$, 
% is a function of $p_\dependency$ and $p_{\instruction}$, where $p_{\dependency}$ and $p_{\instruction}$ are the probabilities of retention of dependency $\dependency$ and instruction $\instruction$ respectively, which can vary with the specific instruction and data-dependency.  
% Details on the probability of sampling $\mathcal{F}_R$, as a function of $p_\dependency$ and $p_{\instruction}$ are in Appendix~\ref{app:pertmodeldetails}. 

% Note that, to preserve all the dependencies $\dependency\in\mathcal{F}_{dep}$ between instructions $\instruction_i$ and $\instruction_j$, $\instruction_i$ and $\instruction_j$ are also preserved by $\Gamma$. 
% This can be seen in $\graphbb$, wherein to preserve a data dependency edge, the corresponding vertices need to be preserved. 
% Thus, $\mathcal{F}_{retained}$ contains the instructions corresponding to all the data dependencies contained in it. 
% However, in order to create some independence between the instructions and data dependencies, $\Gamma$ does not require preservation of the incoming and outgoing data-dependency edges when an instruction needs to be preserved, as $\Gamma$ considers only changes to opcodes of instructions as changes to instructions. 
% Hence, the closed set of features preserved in $\basicblock' = \Gamma(\mathcal{F})$, for a random choice of $\mathcal{F}'_{\costmodel,\basicblock}$  is given by  $\overline{\mathcal{F}'}_{\costmodel,\basicblock} = \mathcal{F}'_{\costmodel,\basicblock}\cup\bigcup_{\dependency_{ij}\in\mathcal{F}_{dep}}\{\instruction_i,\instruction_j\}$.  
% Thus,  $\basicblock'$ is sampled from the identified set $\Hat{\pertmodel}(\overline{\mathcal{F}'}_{\costmodel,\basicblock})$. 

% Thus,  $\basicblock'$ is sampled from the set $\Hat{\pertmodel}(\overline{\mathcal{F}'}_{\costmodel,\basicblock}) \setminus \bigcup_{f\in\Hat{\mathcal{P}}\setminus\overline{\mathcal{F}'}_{\costmodel,\basicblock}}\Hat{\pertmodel}(\overline{\mathcal{F}'}_{\costmodel,\basicblock}\cup\{f\})$. 

% write how it approximates the ideal uniform perturbation distribution

% Every instruction $\instruction\in\mathcal{F}_{changed}$ needs to be either deleted or replaced. 
% Every data dependency $\dependency$ in $\mathcal{F}_{changed}$ must be deleted. 
% thus, every operand $\gamma$ corresponding to $\dependency$ is perturbed to another operand of the same type and size as $\gamma$. The type of $\gamma$ would be memory, register, or immediate/constant, while its size could be a power of $2$ between $2^3-2^9$ bits. 
% Every instruction $\instruction$ in $\mathcal{F}_{changed}$ must be either deleted or replaced with other valid x86 instructions. Let the probability of deletion of $\instruction$ be $p_{del}$. Thus, with probability $p_{del}$, $\Gamma$ deletes $\instruction$ and with $(1-p_{del})$, it replaces its opcode $\omega$ with another opcode that can take the same set of operands as $\omega$ according to the x86 Instruction Set Architecture to get $\basicblock'$. 
% Every data dependency $\dependency\in\Hat{\mathcal{P}}\setminus\overline{\mathcal{F}'}_{\costmodel,\basicblock}$ needs to be deleted. 

% \todo{how well does it approximate uniform distribution?}

% The specific details of \tool{}'s settings for the hyperparameters  $p_{\dependency}$,  $p_{\instruction}$, and $p_{del}$, which allows it to produce roughly uniformly distributed basic blocks are given in Appendix~\ref{app:cometprobset}.
% each element of $\graphbb = (\mathcal{V},\mathcal{E})$, which corresponds to the elements of $\Hat{\mathcal{P}} = \mathcal{V}\cup\mathcal{E}_{dep}\cup\{\lvert\mathcal{V}\rvert\}$ while preserving the features in $\mathcal{F}$. Thus, we perturb $\mathcal{V}$ and $\mathcal{E}_{dep}$ only.  

% \textbf{Perturbing elements of $\mathcal{V}$}.
% Every element $v$ of $\mathcal{V}$ corresponds to an instruction in $\basicblock$. $v$ can be perturbed by either \emph{deleting or replacing} the vertex with another valid vertex. When $v$ is deleted, all incoming and outgoing edges are removed from $\graphbb(\basicblock)$, and a sequence edge is introduced between the vertex preceding and the vertex following $v$. 
% In order to replace $v$, the corresponding instruction $\instruction$'s opcode is replaced with another opcode in the x86 Instruction Set Architecture that can produce a valid x86 instruction with the operands of $\instruction$. This is done so that the resultant $\basicblock'\in\Hat{\pertmodel}(\emptyset)\subseteq B$. We do not change the operands of $\instruction$ for perturbing $v$ as we account for their changes to perturb data dependencies.  
% % changes in operands to be changes in the data-dependency edges in $\graphbb(\basicblock)$ in order to approximately create independence between the graph features. 
% %
% Hence, we independently perturb every $v$ by either deleting it, replacing $v$ with a valid $v'$, or retaining $v$ with equal probability to obtain $\mathcal{V}'$.

% As $\Hat{\mathcal{P}} = \mathcal{V}\cup\mathcal{E}_{dep}\cup\{\lvert\mathcal{V}\rvert\}$, \tool{} consists of custom perturbation algorithms for $\mathcal{V}$ $\mathcal{E}_{dep}\cup\{\lvert\mathcal{V}\rvert  

% \textbf{Perturbing elements of $\mathcal{E}_{dep}$.}
% Every element $\varepsilon$ of $\mathcal{E}_{dep}$,  corresponds to a data-dependency in $\basicblock$. We can perturb $\varepsilon$ by deleting the corresponding dependency. While changes to opcodes of instructions corresponding to the data dependency could result in the deletion of the dependency, we consider their changes vertex perturbations. Hence, we change the operand registers/memory addresses to other registers/memory addresses to break the data dependencies. 
%Note that this change in operands can create new data-dependencies in the resulting basic block, but we do not consider these new dependencies as they are not present in $\basicblock$ and hence can not be important features for its throughput predictions. 
%
% Hence we perturb a data-dependency by deleting it. 
% We prioritize the deletion of data-dependency edges in our implementation as they generally result in minor operand changes and prioritizing their deletion can help us expand the high-probability scenario space of our local basic block distribution. We note, however, that \tool{} can tuned not to prioritize the deletion of the edges in order to obtain a narrower local basic block distribution.


% Algorithm~\ref{alg:perturb_bb} in Appendix~\ref{app:pertalgo} presents our algorithm to (conditionally) perturb a given basic block $\basicblock$.

% \tool{} adopts the explanation feature set extraction algorithm from the Anchors' explanation scheme to solve the optimization problem in~\eqref{eq:overallapproxpractical}. 
\textbf{Computing explanations}. With the basic block perturbation algorithm, $Prec(\mathcal{F})$ is estimated using KL-divergence-based confidence intervals~\citep{kllucb} and $Cov(\mathcal{F})$  is estimated by its empirical value, for a given set of features $\mathcal{F}\subseteq\Hat{\mathcal{P}}$. 
Similar to the Anchors' construction, \tool{} iteratively builds its explanation feature set using a beam search wherein the maximum (estimated) precision feature sets at each level are iteratively expanded to larger feature sets till the precision threshold of $(1-\delta)$ is exceeded. The maximum coverage feature set with precision higher than $(1-\delta)$ is given out as \tool{}'s explanation of $\costmodel(\basicblock)$. 

% As the underlying sample space of $\mathcal{D}_{\mathcal{F}}$ is given by the perturbation function $\Hat{\pertmodel}(\mathcal{F})$, we create our samples by perturbing $\basicblock$ according to an approximately uniform distribution and call our sampling algorithm as the \emph{perturbation sampler} [Section~\ref{sec:implementation}].


% \subsection{Overview of \tool{}'s explanation generation process}
% \tool{} explains the predictions of a given cost model $\costmodel$ for a target basic block $\basicblock$ by first deriving the graph of $\basicblock$ and then selecting the set of graph features $\blockfeat$ (a subset of all graph features $\allfeats(\basicblock)$) that has the maximum precision for throughput prediction (Definition~\ref{def:prec}) and maximum coverage (Definition~\ref{def:cov}) over a local distribution of basic blocks around $\basicblock$. 
% \begin{definition}\label{def:prec}
%     (Precision for throughput prediction). The precision for throughput prediction by cost model $\costmodel$ of a set of target basic block features, $\blockfeat$, is the probability of selecting a basic block $\basicblock'$ in a local conditional basic block distribution $\inputdist_\blockfeat$ conditioned on the features in $\blockfeat$, for which cost model $\costmodel$ predicts a throughput value within 1 clock cycle of the throughput prediction for the target basic block $\basicblock$. 
%     \[Prec_{\costmodel,\inputdist_\blockfeat}(\basicblock, \blockfeat) = Pr_{\basicblock'\in\inputdist_\blockfeat}[\costmodel(\basicblock') \in [\costmodel(\basicblock)-0.5, \costmodel(\basicblock)+0.5]]\]
% \end{definition}
% \begin{definition}\label{def:cov}
%     (Coverage). The coverage of a set of target basic block features, $\blockfeat$, is the probability of selecting a basic block $\basicblock'$ in a local basic block distribution, $\inputdist$ around the target basic block $\basicblock$ that contains the features in $\blockfeat$.
%     \[Coverage_{\costmodel,\inputdist}(\basicblock, \blockfeat) = Pr_{\basicblock'\in\inputdist}[\blockfeat\subseteq \allfeats(\basicblock')]\]
% \end{definition}

% $\blockfeat$ which has the maximum precision for throughput prediction and maximum coverage can be considered responsible for the throughput prediction $\costmodel(\basicblock)$ of cost model $\costmodel$ for target basic block $\basicblock$ within the local input distribution $\inputdist$. We reformulate this dual optimization problem and solve it similarly to the Anchors explanation technique~\citep{anchors}. Particularly, we solve the optimization problem~\eqref{eq:optim}, where $1-\delta$ is a user-defined threshold for the precision of throughput prediction desired for $\blockfeat$ given as the explanation for the prediction $\costmodel(\basicblock)$. 
% \begin{equation}\label{eq:optim}
%     \blockfeat^* = \mathop{argmax}_{\blockfeat \mid Prec_{\costmodel,\inputdist_\blockfeat}(\basicblock, \blockfeat) \geq 1-\delta} Coverage_{\costmodel,\inputdist}(\basicblock, \blockfeat)
% \end{equation}
% We solve the optimization problem~\eqref{eq:optim} by a beam-search for the optimal set of graph features $\blockfeat^*$ that can be given as the explanation for $\costmodel(\basicblock)$, similar to the algorithm used for creating Anchor explanations in \cite{anchors}. 



% \subsection{Estimating precision and coverage of graph features}
% To identify the set of graph features $\blockfeat\subseteq\allfeats(\basicblock)$ that have precision for throughput prediction higher than the threshold $1-\delta$ and maximum coverage, we will need to estimate the precision and coverage of several candidate sets of graph features $\blockfeat$. To estimate the precision for throughput prediction of $\blockfeat$, we sample basic blocks from a local distribution of basic blocks having $\blockfeat$, $\inputdist_\blockfeat$, compute their throughput and create an empirical estimate of the precision. Similarly, to estimate the coverage of $\blockfeat$, we sample basic blocks from a local distribution of basic blocks and empirical estimate the probability of having $\blockfeat$ in the sampled basic block. 

% The crucial step to getting a good estimate of the precision and coverage would be the sampling from the local distribution of basic blocks around the target basic block $\basicblock$. We create these samples by perturbing $\basicblock$ and creating another valid (executable) x86 basic block. The magnitude of our perturbation will govern the locality of the distribution of basic blocks and will affect the precision and coverage and also the faithfulness of our explanations to the actual behavior of the cost model $\costmodel$ on $\basicblock$. 

% Next, we describe the major operations in our perturbation algorithm to get a perturbed basic block $\basicblock'$ from $\basicblock$. A perturbation of $\basicblock$ will essentially be a perturbation of the graph of $\basicblock$, $\graphbb(\basicblock)$, which can be conducted by perturbing its graph features. A node of $\graphbb(\basicblock)$ can be perturbed by either deleting it or replacing it with another valid node. An edge of $\graphbb(\basicblock)$ can be perturbed by deleting the edge. The number of nodes in $\graphbb(\basicblock)$ can be perturbed by deleting some nodes. As we solve the optimization problem in~\eqref{eq:optim} as in the Anchors explanation technique, we treat each of our graph features as arms in a multi-armed bandit setting, in order to apply the KL-LUCB algorithm~\citep{kllucb}. This treatment of the graph features requires them not to be retained or perturbed depending on the status of other graph features. We approximately create this independence between the graph features by restricting the analysis of a node to just the opcode of its corresponding instructions, as the operand values decide the dependency edges in $\graphbb(\basicblock)$ and hence we let any perturbations to operands reflect as perturbations to the graph features corresponding to the edges. We elaborate more on this further into this section. 

% \subsubsection{Perturbing a node of $\graphbb(\basicblock)$}
% Every node of $\graphbb(\basicblock)$ corresponds to an instruction in $\basicblock$. The deletion of a node involves the removal of the node and all of its edges from $\graphbb(\basicblock)$ and the introduction of a sequence edge between the node preceding and the node following the deleted node. 
% In order to replace the instruction $\instruction$ corresponding to a given node, we replace its opcode with another opcode in the x86 Instruction Set Architecture which can produce a valid x86 instruction with the operands of $\instruction$. We do not change the operands of $\instruction$, as we consider the changes in operands to be changes in the data-dependency edges in $\graphbb(\basicblock)$ in order to approximately create independence between the graph features. 
% %
% Hence, we either delete a node, replace the node with another valid node or retain the node with equal probability to obtain the nodes of our perturbed basic block's graph. 



% \subsubsection{Summing up: Basic Block Perturbation algorithm}
% Algorithm~\ref{alg:perturb_bb} presents our algorithm to (conditionally) perturb a given basic block $\basicblock$. The perturbation algorithm can create a perturbed basic block graph while preserving a set of nodes $\overline{\nodes}$, a set of data-dependency edges $\overline{\edges}$ and number of nodes (denoted by the boolean $preserve_\numinsts$). If the number of nodes is to be kept constant, then the node deletion operation is forbidden [lines~\ref{alg:numinststart}-\ref{alg:numinstend}]. Then each of the nodes of $\graphbb(\basicblock)$ is perturbed if it is not required to be retained [lines~\ref{alg:nodeperturbstart}-\ref{alg:nodeperturbend}]. Similarly, each data-dependency edge is perturbed if it is not required to be retained [lines~\ref{alg:edgeperturbstart}-\ref{alg:edgeperturbend}] to form the graph of the perturbed basic block $\graphbb(\overline{\basicblock})$ [line~\ref{alg:makepertbb}].



% \subsection{Theoretical analysis of \tool{}}


% probabilities for data-dependencies:
% retention: 0.1 (freezing) + (0.34 + 0.33*0.5)^2*0.9
